FoPro-KD: Fourier Prompted Effective Knowledge Distillation for Long-Tailed Medical Image Recognition

Representational transfer from publicly available models is a promising technique for improving medical image classification, especially in long-tailed datasets with rare diseases. However, existing methods often overlook the frequency-dependent behavior of these models, thereby limiting their effectiveness in transferring representations and generalizations to rare diseases. In this paper, we propose FoPro-KD, a novel framework that leverages the power of frequency patterns learned from frozen pre-trained models to enhance their transferability and compression, presenting a few unique insights: 1) We demonstrate that leveraging representations from publicly available pre-trained models can substantially improve performance, specifically for rare classes, even when utilizing representations from a smaller pre-trained model. 2) We observe that pre-trained models exhibit frequency preferences, which we explore using our proposed Fourier Prompt Generator (FPG), allowing us to manipulate specific frequencies in the input image, enhancing the discriminative representational transfer. 3) By amplifying or diminishing these frequencies in the input image, we enable Effective Knowledge Distillation (EKD). EKD facilitates the transfer of knowledge from pre-trained models to smaller models. Through extensive experiments in long-tailed gastrointestinal image recognition and skin lesion classification, where rare diseases are prevalent, our FoPro-KD framework outperforms existing methods, enabling more accessible medical models for rare disease classification. Code is available at https://github.com/xmed-lab/FoPro-KD.

==> tmi-5.4-Free_Lunch_Models.tex <==
\subsection{Free Lunch model Ablation}
\label{sec:free_lunch_abl}
%%%%%%%%%%%%%%%%%%%%--BEGIN---%%%%%%%%%%%%%%%%%%%%%%
We present an ablation study of full fine-tuning and linear probing of the ``free lunch models'' pre-trained solely on ImageNet without any knowledge from our target task, used with both the naive cross-entropy (CE) and the baseline, BSM~\cite{Ren2020balms}.

As shown in Table~\ref{tbl:abl:ft_lp_abl}, our experiments on linear probing models reveal that linear probing models initialized with MoCoV2 outperform models initialized with supervised ImageNet pre-training, with a performance gain of 2.26\% and 6.83\% on ``Head`` and ``Tail`` accuracy, respectively. This is because MoCoV2 learns competitive generalizable discriminative representations that benefit the tail classes in linear probing. Thus, our approach of leveraging models pre-trained solely on natural images without any prior knowledge from the target dataset proves to be effective.
% in our EKD Free Lunch model ablation study.

On the other hand, full fine-tuning with the naive-cross entropy benefits the head classes more than linear probing with a gain of 25.18\% on the ``Head'' but comes with a performance drop of 12.7\% on the ``Tail'' in comparison with the best-performing linear probing. These models are computationally heavy for full-fine tuning and deployment, having almost two times the number of parameters as the target model (23 million vs 11 million parameters). Therefore, we propose EKD distilling and compressing such generalization capabilities to smaller models.


\begin{table}[htbp!]
\footnotesize
\centering
\caption{Linear Probing (LP) and Fine-Tuning (FT) Accuracy of free lunch models with naive cross-entropy (CE), averaged over 5 runs across the three imbalance factors for the ISIC-LT dataset. The table includes the accuracy of the majority class (``Head''), the accuracy of the minority class (``Tail''), as well as the Matthew Correlation Coefficient (``MCC''), and the accuracy (``Acc'').}
\vspace{-0.5em}
\label{tbl:abl:ft_lp_abl}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lc|cccc}
\toprule
\multicolumn{2}{c}{Setting}
&\multicolumn{4}{c}{Metric (\%)}
\\
\cline{1-2} \cline{3-6}
Method
&Free Lunch
&Head &Tail&MCC&Acc
\\
\hline
LP&Sup-ImageNet& 65.36&\underline{41.89}&48.77&54.96 \\
LP&MoCov2 &67.62&\textbf{48.72}&\underline{49.85}&\underline{55.99}
\\
\hline 
FT & Random &88.23&22.88&49.46&54.63 \\

FT&MoCov2 &89.93&27.6&56.0&60.48\\
FT
&Sup-ImageNet&\textbf{92.8}&35.93&\textbf{62.51}&\textbf{66.34}\\
\bottomrule
\end{tabular}}
\vspace{-1em}
\end{table} 
%%%%%%%%%%%%%%%%%%%%--End---%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
    \centering
\includegraphics[width=\columnwidth ]{Ablation/free_lunch_bar_plots/barplot_free_lunch_BSM.pdf}
    \caption{Bar plots illustrating the Linear Probing and Fine-Tuning Accuracy of free lunch models with baseline (BSM)~\cite{Ren2020balms} across three imbalance factors (1:100, 1:200, and 1:500) for the ISIC-LT dataset.}
    \label{fig:abl_free_lunch_lp_ft}
\end{figure}


In~\Cref{fig:abl_free_lunch_lp_ft}, we show the results of full fine-tuning and linear probing of the free lunch models utilized with the best-performing baseline, BSM~\cite{Ren2020balms}. We observed that the linear probing of the free lunch model (RN50) trained with contrastive learning (MoCov2) works better than the supervised version linear probed. The performance gain is 2.9\%, 1.2\%, and 2.6\% on the head class and 5.4\%, 6.9\%, and 8.2\% on the tail class for the three imbalance factors, respectively. This gain is attributed to the generalizable features from MoCo-v2 as reported previously. However, when fully fine-tuning the weights of the supervised ImageNet with the baseline~\cite{Ren2020balms}, we observed compelling performance over both the head and tail classes compared to fully fine-tuning initialized with MoCov2. The performance gain is 6.8\%, 5.4\%, and 5.4\% on the ``Head'' and 6.9\%, 14.8\%, and 5.6\% on the ``Tail'' for the three imbalance factors, respectively. This gain can be attributed to the supervised ImageNet's weights being already suited for supervision signals. These results are consistent for all three imbalance factors.



Our experiments have shown unsurprisingly that initialization methods play a crucial role in the performance of deep learning models on imbalanced datasets. While we show empirically that linear probing with contrastive learning approaches works best due to their superior generalization capabilities, we find that the supervised ImageNet initialization provided the best initialization performance for full 
fine-tuning of the free lunch model.



==> tmi-5.6-Weight_Initialization_Ablation.tex <==

% \noindent \textbf{Effectiveness of weight initialization} 

% %*****************--BEGIN---******************
\begin{figure}[htbp!]
\centering
\subfigure[ISIC-LT (1:500)]{
\includegraphics[width=.22\textwidth]{Ablation/pre_training_abl/pre_trained_ISIC.png}
}
% \hspace{-2.5em}
\subfigure[HyPerKvasir]{
\includegraphics[width=.22\textwidth]{Ablation/pre_training_abl/pre_trained_Hyper_sgd_2.png}
}
    \caption{Initialization of target models with ImageNet pre-trained weights and random weights for all methods on ISIC-LT and HyperKVasir datasets. The left y-axis represents the performance of models initialized with random weights, while the right y-axis represents the performance of models initialized with ImageNet pre-trained weights.}
\label{fig:weight_init_two_axis}
% \vspace{-0.5em}
\end{figure}
%*****************--END---******************
\subsection{Effectiveness of weight initialization}\label{sec:weight_init}

In \Cref{fig:weight_init_two_axis}, we demonstrate the importance of weight initialization when dealing with long-tail learning. Recent works have mostly ignored such initialization steps in their empirical experiments to provide fair and better convergence analysis. We agree that pre-trained model weights are architecture-dependent and may not be available for smaller models with the rising of large publicly available pre-trained models. However, if the smaller pre-trained model's weights are available, it can offer a compelling starting point, increasing performance by 4.4\% on ``Acc'' of ISIC-LT 1:500 with the baseline, BSM~\cite{Ren2020balms}. Moreover, initialization with pre-trained weights can further increase our FoPro-KD (``Ours'') performance by 5.0\% on ``Acc`` on the ISIC-LT 1:500. Our method conserves the discriminative distribution capability while training through latent projections with EKD and input manipulation with FPG, which is vital for LT problems. We can also notice that BKD~\cite{ZHANG202336_bkd} is minimally affected on the ISIC 1:500 by pre-trained initialization (an increase of 0.61\% on ``Acc''). 


On the HyperKvasir dataset, we observed that the performance of all methods improves when using the same optimization objective as in~\cite{10.1007/978-3-030-87240-3_31_balanced_mixup}, namely stochastic gradient descent (SGD) with a learning rate of 0.01 and a cosine annealing scheduler.


% ******************
\begin{figure}[htbp!]
\centering
\subfigure[SGD (0.1) vs SGD (0.01)]{
\includegraphics[width=.22\textwidth]{Ablation/pre_training_abl/pre_trained_Hyper_sgd_sgd.png}
}
% \hspace{-2.5em}
\subfigure[SGD (0.1) Initialization]{
\includegraphics[width=.22\textwidth]{Ablation/pre_training_abl/pre_trained_Hyper.png}
}
\subfigure[SGD (0.1) vs Adam]{
\includegraphics[width=.22\textwidth]{Ablation/pre_training_abl/pre_trained_Hyper_adam_sgd.png}
}
% \hspace{-2.5em}
\subfigure[Adam Initialization]{
\includegraphics[width=.22\textwidth]{Ablation/pre_training_abl/pre_trained_Hyper_adam.png}
}
    \caption{Comparison of different optimizers and different initialization on the HyperKvasir dataset. (a) and (c) depict experiments with different optimizers, while (b) and (d) represent experiments with different initializations.
}



\label{fig:weight_init_hyper}
% \vspace{-0.5em}
\end{figure}


In~\Cref{fig:weight_init_hyper}, we present additional experiments conducted on the HyperKvasir dataset. In (a), we observe that SGD with a learning rate of 0.1 and cosine annealing scheduler was optimal for random initialization, outperforming the setting proposed in \cite{10.1007/978-3-030-87240-3_31_balanced_mixup} and increasing the baseline performance~\cite{Ren2020balms} by 2.5\% in terms of ``B-Acc''. However, when using ImageNet initialization with SGD 0.1, we observe in (b) a negative impact on performance, possibly due to the high learning rate distorting the pre-trained features. Nevertheless, our proposed Effective Knowledge Distillation (EKD) approach demonstrates its benefits on both random and pre-trained initialization in (b), with a minimal performance drop of 0.61\% on ``Ours'' compared to a 1.65\% drop on the best-performing baseline~\cite{Ren2020balms} in terms of ``B-Acc''. Furthermore, we can notice in (b) that ``Ours'' and the BKD approach~\cite{ZHANG202336_bkd} are minimally affected by random and pre-trained model initialization. This can be attributed to the utilization of knowledge distillation, which helps maintain stability during training and prevents deviation in the target model's performance. Additionally, our results showed that SGD with a learning rate of 0.1 converged to an optimal point more effectively than most methods when using Adam. However, when initializing with pre-trained weights and using Adam, we achieved a mean of ``B-acc'' of 69.9\%. Overall, our proposed method consistently outperformed other approaches across different weight initialization and optimization strategies, demonstrating its effectiveness.




